Interactive Trimming against Evasive Online Data Manipulation Attacks: A Game-Theoretic Approach

With the exponential growth of data and its crucial impact on our lives and decision-making, the integrity of data has become a significant concern. Malicious data poisoning attacks, where false values are injected into the data, can disrupt machine learning processes and lead to severe consequences. To mitigate these attacks, distance-based defenses, such as trimming, have been proposed, but they can be easily evaded by white-box attackers. The evasiveness and effectiveness of poisoning attack strategies are two sides of the same coin, making game theory a promising approach. However, existing game-theoretical models often overlook the complexities of online data poisoning attacks, where strategies must adapt to the dynamic process of data collection. In this paper, we present an interactive game-theoretical model to defend online data manipulation attacks using the trimming strategy. Our model accommodates a complete strategy space, making it applicable to strong evasive and colluding adversaries. Leveraging the principle of least action and the Euler-Lagrange equation from theoretical physics, we derive an analytical model for the game-theoretic process. To demonstrate its practical usage, we present a case study in a privacy-preserving data collection system under local differential privacy where a non-deterministic utility function is adopted. Two strategies are devised from this analytical model, namely, Tit-for-tat and Elastic. We conduct extensive experiments on real-world datasets, which showcase the effectiveness and accuracy of these two strategies.

==> Elastictriggerstrategy.tex <==
\subsection{Elastic Trigger Strategy}
\label{Elastic Trigger Strategy}
%penalty
%with Forgiveness
%U(u1,u2,du1/dr,du2/dr)的关系：d(u1-u2)/dr=u1-u2
%平移迭加振动

==> Endlessfinite.tex <==
\section{Endless Collection of Finite Samples}
\label{Endlessfinite}

==> Endlessinfinite.tex <==
\section{Endless Collection of Infinite Samples}
\label{Endlessinfinite}
\subsection{Fundamental Settings}
We will borrow the principle of least action from analytical mechanics to describe this system. In the context of this chapter, we will collect an infinite number of samples in an infinite number of rounds, where the number of samples collected in each round is fixed. Therefore, r can be considered as continuum. Furthermore, we will view r as a kind of timer, corresponding to the role of time t in classical mechanics. 

The utility of both sides $u_a$ and $u_c$ are cumulative effects of $r$.

naturally general coordinates

The evolution spatiotemporal structure as 


%稳态解
%Tit for tat
\subsection{Analytical Model}
\begin{Proposition}
The game-theoretical can be denoted by a least action defined by

where $u_a$ and $u_c$ are generalized coordinate
\end{Proposition}

Therefore, we have

\begin{Corollary}
a
\end{Corollary}

\subsection{Equilibrium State}

There is no interaction between . Therefore, the Lagrangian is additive. 

\begin{Proposition}
The Lagrangian of a Nash Equilibrium state can be written as
\begin{equation}
\mathcal{L}=m_a\dot{u_a}^2+m_c\dot{u_c}^2
\end{equation}
\end{Proposition}


%纳什均衡应该是一个稳态
%二者在稳态时没有相互作用，因此拉格朗日函数可加，对r和u都均匀，不显含r和u
%L=L(v^2), du/dt=const

